Vibe Coding in Software Development: A Multivocal Literature Review

Vibe coding is an AI-assisted software development approach in which developers express intent in natural language and large language models generate code. To our knowledge, no review has synthesized academic and practitioner sources under a common protocol. We conducted a multivocal literature review of publications from January 2022 to 9 September 2026, identified through searches in October 2025 and September 2026. After assessing source quality and credibility, we analyzed 266 sources (76 peer-reviewed, 190 grey) across eight research questions: 146 were direct, 93 adjacent, and 27 background. Presence and outcome findings receive reporting-support and evidence-strength labels, respectively. The second author conducted twelve checks; pre-reconciliation agreement was low in several, but substantial for the final directness rule and moderate for the outcome fields, which were checked in full. Sources describe a generation-evaluation-revision loop, with developer work shifting from writing code toward directing, supervising, and validating. Productivity is reported in 109 of the 159 sources contributing to the outcome question, of which 22 provide assertions only; these counts indicate reporting, not effect size. Most comparable sources report short-term productivity gains and long-term maintainability costs, but both receive Weak evidence-strength labels because some comparable sources report opposing directions. Short-term quality and defects are labeled Weak. Long-term productivity, long-term quality, and short-term reproducibility are labeled Moderate. Prototyping is reported more often than production use, and user-interface work more often than data and machine-learning work, but task-domain evidence is sparse. Future work should evaluate safeguards, session-level dynamics, long-term maintainability, and production use.

==> tab_app_evidence_assignment.tex <==
\begingroup\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.1}\captionsetup{font={sf,small},labelfont={bf},labelsep=newline,justification=justified,singlelinecheck=false}
\begin{longtable}{|p{0.95cm}|p{3.5cm}|p{1.4cm}|p{0.6cm}|p{0.6cm}|p{0.6cm}|p{0.6cm}|p{1.3cm}|p{2.2cm}|p{2.1cm}|}
\caption{Label of every finding with its criterion values (Section~\ref{sec:evidence_strength}). Presence findings (RQ1 to RQ3, RQ5 to RQ8) carry reporting-support labels, and outcome findings (RQ4) evidence-strength labels.}\label{tab:app_evidence_assignment}\\
\hline\rowcolor[HTML]{EFEFEF}\textbf{RQ} & \textbf{Finding} & \textbf{Horizon} & \textbf{n} & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{Restricted share} & \textbf{C4} & \textbf{Label} \\\hline\endfirsthead
\hline\rowcolor[HTML]{EFEFEF}\textbf{RQ} & \textbf{Finding} & \textbf{Horizon} & \textbf{n} & \textbf{C1} & \textbf{C2} & \textbf{C3} & \textbf{Restricted share} & \textbf{C4} & \textbf{Label} \\\hline\endhead
RQ1 & Agentic or semi-autonomous development & all & 78 & 76 & 13 & 26 & 21\% & not applicable & Strong reporting support \\
\hline
RQ1 & AI-assisted development & all & 50 & 50 & 10 & 13 & 20\% & not applicable & Strong reporting support \\
\hline
RQ1 & AI-native IDE & all & 10 & 10 & 3 & 3 & 20\% & not applicable & Strong reporting support \\
\hline
RQ1 & End-user or non-programmer development & all & 33 & 33 & 7 & 8 & 36\% & not applicable & Moderate reporting support \\
\hline
RQ1 & Natural-language-to-code or prompt-based development & all & 159 & 155 & 38 & 45 & 22\% & not applicable & Strong reporting support \\
\hline
RQ1 & Socio-technical practice & all & 137 & 131 & 15 & 39 & 34\% & not applicable & Moderate reporting support \\
\hline
RQ2 & Chat-based iterative development loop & all & 50 & 50 & 11 & 14 & 0\% & not applicable & Strong reporting support \\
\hline
RQ2 & Explicit context provisioning & all & 75 & 73 & 12 & 31 & 0\% & not applicable & Strong reporting support \\
\hline
RQ2 & Validation and evaluation pipelines as a core loop & all & 69 & 67 & 12 & 31 & 0\% & not applicable & Strong reporting support \\
\hline
RQ2 & Inline IDE-assisted completion & all & 3 & 3 & 1 & 0 & 0\% & not applicable & Weak reporting support \\
\hline
RQ2 & Iterate-prompt-patch loop & all & 96 & 94 & 22 & 33 & 0\% & not applicable & Strong reporting support \\
\hline
RQ2 & Patch and repair workflow & all & 26 & 25 & 3 & 11 & 0\% & not applicable & Strong reporting support \\
\hline
RQ2 & Collaborative prompt practices & all & 7 & 7 & 3 & 1 & 0\% & not applicable & Moderate reporting support \\
\hline
RQ2 & Retrieval and documentation grounding & all & 8 & 8 & 3 & 1 & 0\% & not applicable & Strong reporting support \\
\hline
RQ3.1 & Shift from direct authoring toward supervision and steering roles & all & 56 & 55 & 10 & 22 & 0\% & not applicable & Strong reporting support \\
\hline
RQ3.1 & Cognitive debt due to deferred understanding & all & 32 & 31 & 9 & 6 & 0\% & not applicable & Strong reporting support \\
\hline
RQ3.1 & Changes in cognitive load & all & 66 & 65 & 19 & 22 & 0\% & not applicable & Strong reporting support \\
\hline
RQ3.1 & Flow effects & all & 22 & 22 & 8 & 4 & 0\% & not applicable & Strong reporting support \\
\hline
RQ3.1 & Trust calibration and adaptive reliance & all & 86 & 82 & 22 & 29 & 0\% & not applicable & Strong reporting support \\
\hline
RQ3.2 & Context window or state-retention failures & all & 35 & 35 & 12 & 13 & 0\% & not applicable & Strong reporting support \\
\hline
RQ3.2 & Repetitive prompt-patch cycles without convergence & all & 44 & 43 & 14 & 14 & 0\% & not applicable & Strong reporting support \\
\hline
RQ3.2 & Session momentum breaks due to failure, misalignment, or tool friction & all & 26 & 26 & 8 & 7 & 0\% & not applicable & Strong reporting support \\
\hline
RQ3.3 & Expert acceleration & all & 54 & 52 & 14 & 15 & 0\% & not applicable & Strong reporting support \\
\hline
RQ3.3 & Novice or non-programmer orientation & all & 88 & 85 & 29 & 28 & 0\% & not applicable & Strong reporting support \\
\hline
RQ3.3 & Data and machine learning tasks & all & 5 & 5 & 1 & 2 & 0\% & not applicable & Moderate reporting support \\
\hline
RQ3.3 & UI and front-end tasks & all & 12 & 12 & 2 & 5 & 0\% & not applicable & Moderate reporting support \\
\hline
RQ4 & Defect risks and error patterns & short-term & 43 & 42 & 6 & 20 & 0\% & contested & Weak evidence \\
\hline
RQ4 & Defect risks and error patterns & long-term & 5 & 5 & 0 & 0 & 0\% & not assessable & Weak evidence \\
\hline
RQ4 & Maintainability implications & short-term & 3 & 3 & 1 & 0 & 0\% & not assessable & Weak evidence \\
\hline
RQ4 & Maintainability implications & long-term & 35 & 33 & 6 & 13 & 0\% & contested & Weak evidence \\
\hline
RQ4 & Productivity & short-term & 105 & 101 & 27 & 29 & 0\% & contested & Weak evidence \\
\hline
RQ4 & Productivity & long-term & 8 & 8 & 5 & 1 & 0\% & minor disagreement & Moderate evidence \\
\hline
RQ4 & Code or UI quality & short-term & 88 & 86 & 22 & 40 & 0\% & contested & Weak evidence \\
\hline
RQ4 & Code or UI quality & long-term & 8 & 8 & 1 & 2 & 0\% & minor disagreement & Moderate evidence \\
\hline
RQ4 & Reproducibility and consistency & short-term & 7 & 7 & 1 & 2 & 0\% & consistent & Moderate evidence \\
\hline
RQ5.1 & Cumulative context errors and iteration drift & all & 33 & 33 & 5 & 15 & 0\% & not applicable & Strong reporting support \\
\hline
RQ5.1 & Hallucinations and incorrect generations & all & 100 & 96 & 28 & 36 & 0\% & not applicable & Strong reporting support \\
\hline
RQ5.1 & Licensing and provenance uncertainty & all & 7 & 7 & 1 & 2 & 0\% & not applicable & Moderate reporting support \\
\hline
RQ5.1 & Minimal-review commits and insufficient inspection practices & all & 25 & 24 & 5 & 9 & 0\% & not applicable & Strong reporting support \\
\hline
RQ5.1 & Brittle prompts and prompt sensitivity & all & 27 & 26 & 5 & 14 & 0\% & not applicable & Strong reporting support \\
\hline
RQ5.2 & Explicit guidance on when to avoid vibe coding & all & 20 & 19 & 9 & 4 & 0\% & not applicable & Strong reporting support \\
\hline
RQ5.2 & Human-in-the-loop review & all & 108 & 105 & 31 & 36 & 0\% & not applicable & Strong reporting support \\
\hline
RQ5.2 & Provenance tracking and traceability mechanisms & all & 23 & 23 & 7 & 7 & 0\% & not applicable & Strong reporting support \\
\hline
RQ5.2 & Sandboxing and constrained execution environments & all & 12 & 12 & 3 & 2 & 0\% & not applicable & Strong reporting support \\
\hline
RQ5.2 & Validation and testing pipelines & all & 109 & 107 & 29 & 42 & 0\% & not applicable & Strong reporting support \\
\hline
RQ6 & Cost or usage-limit constraints & all & 21 & 21 & 3 & 8 & 0\% & not applicable & Strong reporting support \\
\hline
RQ6 & Privacy or exposure of data and code & all & 26 & 25 & 6 & 7 & 0\% & not applicable & Strong reporting support \\
\hline
RQ6 & Use in production or operational deployment contexts & all & 41 & 41 & 15 & 7 & 0\% & not applicable & Strong reporting support \\
\hline
RQ6 & Use in prototyping or early-stage development contexts & all & 55 & 55 & 17 & 13 & 0\% & not applicable & Strong reporting support \\
\hline
RQ7 & Coding agents and agent modes & all & 74 & 73 & 8 & 27 & 24\% & not applicable & Strong reporting support \\
\hline
RQ7 & ChatGPT and OpenAI models & all & 101 & 98 & 23 & 35 & 15\% & not applicable & Strong reporting support \\
\hline
RQ7 & Claude and Anthropic tools & all & 131 & 129 & 25 & 39 & 27\% & not applicable & Moderate reporting support \\
\hline
RQ7 & GitHub Copilot & all & 73 & 72 & 19 & 19 & 15\% & not applicable & Strong reporting support \\
\hline
RQ7 & Cursor & all & 95 & 92 & 20 & 23 & 29\% & not applicable & Moderate reporting support \\
\hline
RQ7 & Evaluation frameworks and benchmarks & all & 14 & 14 & 4 & 10 & 7\% & not applicable & Strong reporting support \\
\hline
RQ8 & Context management limitations & all & 21 & 21 & 3 & 10 & 0\% & not applicable & Strong reporting support \\
\hline
RQ8 & Lack of standardized evaluation and benchmarks & all & 69 & 68 & 20 & 34 & 0\% & not applicable & Strong reporting support \\
\hline
RQ8 & Governance, disclosure, and organizational integration challenges & all & 12 & 12 & 3 & 4 & 0\% & not applicable & Strong reporting support \\
\hline
RQ8 & Security concerns including unsafe code, vulnerabilities, and misuse risks & all & 14 & 14 & 4 & 6 & 0\% & not applicable & Strong reporting support \\
\hline
RQ8 & Trust, misuse, and reliability challenges & all & 22 & 21 & 7 & 10 & 0\% & not applicable & Strong reporting support \\
\hline
\end{longtable}
\noindent{\footnotesize n = sources coded with the finding after background sources are set aside and non-supporting candidates are removed. The results tables report the count before these steps, so n can be smaller. C4 for the outcome findings (RQ4) follows the direction rule of Section~\ref{sec:evidence_strength} and is not assessable when fewer than two comparable sources record a direction. For the other findings, which record that a phenomenon is reported and carry no direction, C4 is not applicable. The supporting source ids of every finding are in the replication package.}\par
\endgroup


==> tab_app_subsets.tex <==
\begingroup\scriptsize\setlength{\tabcolsep}{3pt}\renewcommand{\arraystretch}{1.1}\captionsetup{font={sf,small},labelfont={bf},labelsep=newline,justification=justified,singlelinecheck=false}
\begin{longtable}{|p{0.75cm}|p{2.39cm}|p{1.13cm}|p{1.22cm}|p{1.22cm}|p{1.22cm}|p{1.22cm}|p{1.22cm}|p{1.22cm}|p{1.22cm}|p{1.22cm}|}
\caption{Label of every finding on the full corpus and on each subset. For presence findings (RQ1 to RQ3, RQ5 to RQ8) the label is reporting support, and for outcome findings (RQ4) it is evidence strength.}\label{tab:app_subsets}\\
\hline\rowcolor[HTML]{EFEFEF}\textbf{RQ} & \textbf{Finding} & \textbf{Horizon} & \textbf{Full} & \textbf{Direct} & \textbf{No Tier~3} & \textbf{No restricted cat.} & \textbf{Window 1 only} & \textbf{Window 2 only} & \textbf{No merging} & \textbf{Direct by term} \\\hline\endfirsthead
\hline\rowcolor[HTML]{EFEFEF}\textbf{RQ} & \textbf{Finding} & \textbf{Horizon} & \textbf{Full} & \textbf{Direct} & \textbf{No Tier~3} & \textbf{No restricted cat.} & \textbf{Window 1 only} & \textbf{Window 2 only} & \textbf{No merging} & \textbf{Direct by term} \\\hline\endhead
RQ1 & Agentic or semi-autonomous development & all & Strong & Moderate & Strong & Strong & Moderate & Strong & Strong & Moderate \\
\hline
RQ1 & AI-assisted development & all & Strong & Moderate & Strong & Strong & Moderate & Strong & Strong & Moderate \\
\hline
RQ1 & AI-native IDE & all & Strong & Weak & Strong & Strong & Moderate & Moderate & Strong & Weak \\
\hline
RQ1 & End-user or non-programmer development & all & Moderate & Moderate & Moderate & Strong & Moderate & Moderate & Moderate & Moderate \\
\hline
RQ1 & Natural-language-to-code or prompt-based development & all & Strong & Moderate & Strong & Strong & Moderate & Strong & Strong & Moderate \\
\hline
RQ1 & Socio-technical practice & all & Moderate & Moderate & Strong & Strong & Moderate & Moderate & Moderate & Moderate \\
\hline
RQ2 & Chat-based iterative development loop & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ2 & Explicit context provisioning & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
RQ2 & Validation and evaluation pipelines as a core loop & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ2 & Inline IDE-assisted completion & all & Weak & Emerging & Weak & Weak & Emerging & Emerging & Weak & Emerging \\
\hline
RQ2 & Iterate-prompt-patch loop & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ2 & Patch and repair workflow & all & Strong & Moderate & Strong & Strong & Moderate & Moderate & Strong & Moderate \\
\hline
RQ2 & Collaborative prompt practices & all & Moderate & Moderate & Moderate & Moderate & Emerging & Moderate & Moderate & Moderate \\
\hline
RQ2 & Retrieval and documentation grounding & all & Strong & Weak & Strong & Strong & Strong & no support & Strong & Weak \\
\hline
RQ3.1 & Shift from direct authoring toward supervision and steering roles & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ3.1 & Cognitive debt due to deferred understanding & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
RQ3.1 & Changes in cognitive load & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ3.1 & Flow effects & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ3.1 & Trust calibration and adaptive reliance & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ3.2 & Context window or state-retention failures & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
RQ3.2 & Repetitive prompt-patch cycles without convergence & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ3.2 & Session momentum breaks due to failure, misalignment, or tool friction & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ3.3 & Expert acceleration & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
RQ3.3 & Novice or non-programmer orientation & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ3.3 & Data and machine learning tasks & all & Moderate & Weak & Moderate & Moderate & Emerging & Weak & Moderate & Weak \\
\hline
RQ3.3 & UI and front-end tasks & all & Moderate & Moderate & Moderate & Moderate & Weak & Moderate & Moderate & Moderate \\
\hline
RQ4 & Defect risks and error patterns & short-term & Weak & Moderate & Weak & Weak & Moderate & Weak & Weak & Moderate \\
\hline
RQ4 & Defect risks and error patterns & long-term & Weak & Weak & Weak & Weak & Weak & Weak & Weak & Weak \\
\hline
RQ4 & Maintainability implications & short-term & Weak & Weak & Weak & Weak & Weak & Weak & Weak & Weak \\
\hline
RQ4 & Maintainability implications & long-term & Weak & Moderate & Weak & Weak & Moderate & Weak & Weak & Moderate \\
\hline
RQ4 & Productivity & short-term & Weak & Weak & Weak & Weak & Moderate & Weak & Weak & Weak \\
\hline
RQ4 & Productivity & long-term & Moderate & Moderate & Moderate & Moderate & Weak & Moderate & Moderate & Moderate \\
\hline
RQ4 & Code or UI quality & short-term & Weak & Weak & Weak & Weak & Weak & Weak & Weak & Weak \\
\hline
RQ4 & Code or UI quality & long-term & Moderate & Weak & Moderate & Moderate & Weak & Moderate & Moderate & Weak \\
\hline
RQ4 & Reproducibility and consistency & short-term & Moderate & Weak & Moderate & Moderate & Moderate & no support & Moderate & Weak \\
\hline
RQ5.1 & Cumulative context errors and iteration drift & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
RQ5.1 & Hallucinations and incorrect generations & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ5.1 & Licensing and provenance uncertainty & all & Moderate & Emerging & Moderate & Moderate & Weak & Weak & Moderate & Emerging \\
\hline
RQ5.1 & Minimal-review commits and insufficient inspection practices & all & Strong & Strong & Strong & Strong & Weak & Strong & Strong & Strong \\
\hline
RQ5.1 & Brittle prompts and prompt sensitivity & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
RQ5.2 & Explicit guidance on when to avoid vibe coding & all & Strong & Strong & Strong & Strong & Emerging & Strong & Strong & Strong \\
\hline
RQ5.2 & Human-in-the-loop review & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ5.2 & Provenance tracking and traceability mechanisms & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
RQ5.2 & Sandboxing and constrained execution environments & all & Strong & Moderate & Strong & Strong & Moderate & Moderate & Strong & Moderate \\
\hline
RQ5.2 & Validation and testing pipelines & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ6 & Cost or usage-limit constraints & all & Strong & Moderate & Strong & Strong & Strong & Moderate & Strong & Moderate \\
\hline
RQ6 & Privacy or exposure of data and code & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
RQ6 & Use in production or operational deployment contexts & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
RQ6 & Use in prototyping or early-stage development contexts & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ7 & Coding agents and agent modes & all & Strong & Moderate & Strong & Strong & Moderate & Strong & Strong & Moderate \\
\hline
RQ7 & ChatGPT and OpenAI models & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
RQ7 & Claude and Anthropic tools & all & Moderate & Moderate & Strong & Strong & Moderate & Strong & Moderate & Moderate \\
\hline
RQ7 & GitHub Copilot & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
RQ7 & Cursor & all & Moderate & Moderate & Strong & Strong & Moderate & Strong & Moderate & Moderate \\
\hline
RQ7 & Evaluation frameworks and benchmarks & all & Strong & Emerging & Strong & Strong & Weak & Strong & Strong & Emerging \\
\hline
RQ8 & Context management limitations & all & Strong & Moderate & Strong & Strong & Moderate & Moderate & Strong & Moderate \\
\hline
RQ8 & Lack of standardized evaluation and benchmarks & all & Strong & Strong & Strong & Strong & Strong & Strong & Strong & Strong \\
\hline
RQ8 & Governance, disclosure, and organizational integration challenges & all & Strong & Moderate & Strong & Strong & Moderate & Moderate & Strong & Moderate \\
\hline
RQ8 & Security concerns including unsafe code, vulnerabilities, and misuse risks & all & Strong & Moderate & Strong & Strong & Moderate & Moderate & Strong & Moderate \\
\hline
RQ8 & Trust, misuse, and reliability challenges & all & Strong & Strong & Strong & Strong & Moderate & Strong & Strong & Strong \\
\hline
\end{longtable}
\endgroup


==> tab_app_thresholds.tex <==

\begin{table*}[!t]
\centering
\footnotesize
\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{4pt}
\caption{Threshold sensitivity: findings whose label changes when one threshold of the matrix is moved by one step, the others fixed, and the effect of a minority-share variant of the C4 rule.}
\label{tab:app_thresholds}
\begin{tabular}{|p{4.2cm}|p{12.4cm}|}
\hline
\rowcolor[HTML]{EFEFEF}
\textbf{Threshold moved} & \textbf{Findings whose label changes} \\
\hline
Strong: at least 8 independent sources, moved to 7 & RQ2 Collaborative prompt practices: Moderate to Strong \\
\hline
Strong: at least 8 independent sources, moved to 9 & RQ2 Retrieval and documentation grounding: Strong to Moderate \\
\hline
Strong: at least 3 comparable peer-reviewed studies, moved to 2 & RQ3.3 UI and front-end tasks: Moderate to Strong \\
\hline
Strong: at least 3 comparable peer-reviewed studies, moved to 4 & RQ1 AI-native IDE: Strong to Moderate; RQ2 Patch and repair workflow: Strong to Moderate; RQ2 Retrieval and documentation grounding: Strong to Moderate; RQ5.2 Sandboxing and constrained execution environments: Strong to Moderate; RQ6 Cost or usage-limit constraints: Strong to Moderate; RQ8 Context management limitations: Strong to Moderate; RQ8 Governance, disclosure, and organizational integration challenges: Strong to Moderate \\
\hline
Moderate: at least 5 independent sources, moved to 4 & none \\
\hline
Moderate: at least 5 independent sources, moved to 6 & RQ3.3 Data and machine learning tasks: Moderate to Weak \\
\hline
Moderate: at least 2 comparable grey sources, moved to 1 & none \\
\hline
Moderate: at least 2 comparable grey sources, moved to 3 & none \\
\hline
Strong: restricted share below 25\%, moved to 20\% & RQ1 Agentic or semi-autonomous development: Strong to Moderate; RQ1 AI-assisted development: Strong to Moderate; RQ1 AI-native IDE: Strong to Moderate; RQ1 Natural-language-to-code or prompt-based development: Strong to Moderate; RQ7 Coding agents and agent modes: Strong to Moderate \\
\hline
Strong: restricted share below 25\%, moved to 30\% & RQ7 Claude and Anthropic tools: Moderate to Strong; RQ7 Cursor: Moderate to Strong \\
\hline
C4: contested when one comparable source opposes, moved to contested only when the minority is at least 20\% & RQ4 Defect risks and error patterns short-term: Weak to Moderate; RQ4 Maintainability implications long-term: Weak to Moderate; RQ4 Productivity short-term: Weak to Moderate \\
\hline
\end{tabular}
\end{table*}


==> tab_rq4_by_design.tex <==

\begingroup\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.1}\captionsetup{font={sf,small},labelfont={bf},labelsep=newline,justification=justified,singlelinecheck=false}
\begin{longtable}{|p{2.14cm}|p{1.34cm}|p{1.70cm}|p{3.21cm}|p{0.62cm}|p{1.87cm}|p{1.87cm}|p{2.14cm}|}
\caption{RQ4 outcome rows by stream and study design. Peer-reviewed sources are grouped by method and grey sources by evidence category. Directions are given as positive / negative / mixed / no effect. Background and restricted sources are not counted.}\label{tab:rq4_by_design}\\
\hline\rowcolor[HTML]{EFEFEF}\textbf{Outcome} & \textbf{Horizon} & \textbf{Stream} & \textbf{Design group} & \textbf{n} & \textbf{Positive / negative / mixed / no effect, comparable sources} & \textbf{Positive / negative / mixed / no effect, other sources} & \textbf{Measured / self-reported / asserted} \\\hline\endfirsthead
\hline\rowcolor[HTML]{EFEFEF}\textbf{Outcome} & \textbf{Horizon} & \textbf{Stream} & \textbf{Design group} & \textbf{n} & \textbf{Positive / negative / mixed / no effect, comparable sources} & \textbf{Positive / negative / mixed / no effect, other sources} & \textbf{Measured / self-reported / asserted} \\\hline\endhead
Productivity & short-term & peer-reviewed & Benchmark & 1 & 0 / 0 / 1 / 0 & 0 / 0 / 0 / 0 & 1 / 0 / 0 \\
\hline
Productivity & short-term & peer-reviewed & Case study & 8 & 2 / 0 / 2 / 0 & 2 / 0 / 1 / 0 & 4 / 4 / 0 \\
\hline
Productivity & short-term & peer-reviewed & Design proposal or tool description & 3 & 1 / 0 / 0 / 0 & 1 / 0 / 1 / 0 & 2 / 0 / 1 \\
\hline
Productivity & short-term & peer-reviewed & Experiment or user study & 2 & 1 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 1 / 1 / 0 \\
\hline
Productivity & short-term & peer-reviewed & Interviews & 3 & 2 / 0 / 1 / 0 & 0 / 0 / 0 / 0 & 0 / 3 / 0 \\
\hline
Productivity & short-term & peer-reviewed & Mixed methods & 6 & 3 / 0 / 1 / 1 & 1 / 0 / 0 / 0 & 5 / 1 / 0 \\
\hline
Productivity & short-term & peer-reviewed & Not reported & 1 & 0 / 0 / 0 / 0 & 0 / 0 / 1 / 0 & 0 / 1 / 0 \\
\hline
Productivity & short-term & peer-reviewed & Other & 6 & 2 / 0 / 2 / 0 & 2 / 0 / 0 / 0 & 1 / 2 / 3 \\
\hline
Productivity & short-term & peer-reviewed & Repository mining & 4 & 1 / 1 / 1 / 1 & 0 / 0 / 0 / 0 & 3 / 1 / 0 \\
\hline
Productivity & short-term & peer-reviewed & Static or automated analysis & 3 & 1 / 0 / 0 / 0 & 2 / 0 / 0 / 0 & 1 / 0 / 2 \\
\hline
Productivity & short-term & peer-reviewed & Survey & 2 & 0 / 0 / 0 / 1 & 1 / 0 / 0 / 0 & 1 / 1 / 0 \\
\hline
Productivity & short-term & grey & Conceptual & 7 & 0 / 0 / 0 / 0 & 3 / 1 / 3 / 0 & 4 / 1 / 2 \\
\hline
Productivity & short-term & grey & Empirical & 19 & 14 / 1 / 3 / 1 & 0 / 0 / 0 / 0 & 8 / 10 / 1 \\
\hline
Productivity & short-term & grey & Experience report & 17 & 0 / 0 / 0 / 0 & 14 / 0 / 3 / 0 & 3 / 12 / 2 \\
\hline
Productivity & short-term & grey & Position & 3 & 0 / 0 / 0 / 0 & 1 / 1 / 1 / 0 & 0 / 1 / 2 \\
\hline
Productivity & short-term & grey & Secondary & 10 & 0 / 0 / 0 / 0 & 7 / 1 / 2 / 0 & 2 / 2 / 6 \\
\hline
Productivity & short-term & grey & Tool/System & 10 & 7 / 0 / 3 / 0 & 0 / 0 / 0 / 0 & 5 / 2 / 3 \\
\hline
Productivity & long-term & peer-reviewed & Case study & 1 & 0 / 0 / 1 / 0 & 0 / 0 / 0 / 0 & 1 / 0 / 0 \\
\hline
Productivity & long-term & peer-reviewed & Interviews & 1 & 0 / 0 / 1 / 0 & 0 / 0 / 0 / 0 & 0 / 1 / 0 \\
\hline
Productivity & long-term & peer-reviewed & Other & 2 & 0 / 0 / 2 / 0 & 0 / 0 / 0 / 0 & 0 / 2 / 0 \\
\hline
Productivity & long-term & peer-reviewed & Repository mining & 1 & 0 / 0 / 1 / 0 & 0 / 0 / 0 / 0 & 1 / 0 / 0 \\
\hline
Productivity & long-term & grey & Empirical & 1 & 0 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 1 / 0 / 0 \\
\hline
Productivity & long-term & grey & Experience report & 2 & 0 / 0 / 0 / 0 & 0 / 0 / 2 / 0 & 1 / 1 / 0 \\
\hline
Code or UI quality & short-term & peer-reviewed & Benchmark & 4 & 0 / 2 / 2 / 0 & 0 / 0 / 0 / 0 & 4 / 0 / 0 \\
\hline
Code or UI quality & short-term & peer-reviewed & Case study & 6 & 0 / 2 / 3 / 0 & 0 / 0 / 1 / 0 & 3 / 3 / 0 \\
\hline
Code or UI quality & short-term & peer-reviewed & Experiment or user study & 2 & 0 / 0 / 2 / 0 & 0 / 0 / 0 / 0 & 1 / 1 / 0 \\
\hline
Code or UI quality & short-term & peer-reviewed & Mixed methods & 9 & 2 / 3 / 3 / 0 & 0 / 1 / 0 / 0 & 7 / 2 / 0 \\
\hline
Code or UI quality & short-term & peer-reviewed & Other & 1 & 0 / 0 / 1 / 0 & 0 / 0 / 0 / 0 & 0 / 1 / 0 \\
\hline
Code or UI quality & short-term & peer-reviewed & Repository mining & 1 & 0 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 0 / 1 / 0 \\
\hline
Code or UI quality & short-term & peer-reviewed & Static or automated analysis & 2 & 0 / 1 / 0 / 0 & 0 / 0 / 1 / 0 & 0 / 1 / 1 \\
\hline
Code or UI quality & short-term & grey & Conceptual & 3 & 0 / 0 / 0 / 0 & 1 / 2 / 0 / 0 & 0 / 1 / 2 \\
\hline
Code or UI quality & short-term & grey & Empirical & 23 & 2 / 5 / 15 / 0 & 0 / 0 / 0 / 0 & 17 / 5 / 1 \\
\hline
Code or UI quality & short-term & grey & Experience report & 14 & 0 / 0 / 0 / 0 & 4 / 2 / 8 / 0 & 2 / 10 / 2 \\
\hline
Code or UI quality & short-term & grey & Position & 2 & 0 / 0 / 0 / 0 & 0 / 2 / 0 / 0 & 1 / 0 / 1 \\
\hline
Code or UI quality & short-term & grey & Secondary & 4 & 0 / 0 / 0 / 0 & 1 / 2 / 1 / 0 & 3 / 0 / 1 \\
\hline
Code or UI quality & short-term & grey & Tool/System & 17 & 9 / 1 / 7 / 0 & 0 / 0 / 0 / 0 & 14 / 1 / 2 \\
\hline
Code or UI quality & long-term & peer-reviewed & Repository mining & 1 & 0 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 1 / 0 / 0 \\
\hline
Code or UI quality & long-term & peer-reviewed & Static or automated analysis & 1 & 0 / 0 / 0 / 0 & 0 / 0 / 1 / 0 & 0 / 0 / 1 \\
\hline
Code or UI quality & long-term & grey & Empirical & 2 & 0 / 0 / 0 / 2 & 0 / 0 / 0 / 0 & 2 / 0 / 0 \\
\hline
Code or UI quality & long-term & grey & Experience report & 3 & 0 / 0 / 0 / 0 & 0 / 0 / 3 / 0 & 0 / 2 / 1 \\
\hline
Code or UI quality & long-term & grey & Position & 1 & 0 / 0 / 0 / 0 & 0 / 1 / 0 / 0 & 0 / 0 / 1 \\
\hline
Defect risks and error patterns & short-term & peer-reviewed & Benchmark & 2 & 0 / 2 / 0 / 0 & 0 / 0 / 0 / 0 & 2 / 0 / 0 \\
\hline
Defect risks and error patterns & short-term & peer-reviewed & Case study & 1 & 0 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 1 / 0 / 0 \\
\hline
Defect risks and error patterns & short-term & peer-reviewed & Design proposal or tool description & 1 & 0 / 0 / 0 / 0 & 0 / 1 / 0 / 0 & 0 / 0 / 1 \\
\hline
Defect risks and error patterns & short-term & peer-reviewed & Mixed methods & 1 & 0 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 0 / 1 / 0 \\
\hline
Defect risks and error patterns & short-term & peer-reviewed & Other & 2 & 0 / 0 / 1 / 0 & 1 / 0 / 0 / 0 & 0 / 1 / 1 \\
\hline
Defect risks and error patterns & short-term & peer-reviewed & Repository mining & 1 & 0 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 1 / 0 / 0 \\
\hline
Defect risks and error patterns & short-term & grey & Conceptual & 4 & 0 / 0 / 0 / 0 & 0 / 3 / 1 / 0 & 1 / 0 / 3 \\
\hline
Defect risks and error patterns & short-term & grey & Empirical & 12 & 0 / 8 / 4 / 0 & 0 / 0 / 0 / 0 & 9 / 2 / 1 \\
\hline
Defect risks and error patterns & short-term & grey & Experience report & 7 & 0 / 0 / 0 / 0 & 1 / 4 / 2 / 0 & 2 / 2 / 3 \\
\hline
Defect risks and error patterns & short-term & grey & Position & 3 & 0 / 0 / 0 / 0 & 0 / 2 / 1 / 0 & 1 / 1 / 1 \\
\hline
Defect risks and error patterns & short-term & grey & Secondary & 1 & 0 / 0 / 0 / 0 & 0 / 1 / 0 / 0 & 0 / 0 / 1 \\
\hline
Defect risks and error patterns & short-term & grey & Tool/System & 8 & 2 / 2 / 4 / 0 & 0 / 0 / 0 / 0 & 7 / 0 / 1 \\
\hline
Defect risks and error patterns & long-term & grey & Conceptual & 1 & 0 / 0 / 0 / 0 & 0 / 1 / 0 / 0 & 0 / 1 / 0 \\
\hline
Defect risks and error patterns & long-term & grey & Experience report & 2 & 0 / 0 / 0 / 0 & 0 / 1 / 1 / 0 & 0 / 1 / 1 \\
\hline
Defect risks and error patterns & long-term & grey & Secondary & 2 & 0 / 0 / 0 / 0 & 0 / 2 / 0 / 0 & 1 / 1 / 0 \\
\hline
Maintainability implications & short-term & peer-reviewed & Repository mining & 1 & 0 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 1 / 0 / 0 \\
\hline
Maintainability implications & short-term & grey & Experience report & 2 & 0 / 0 / 0 / 0 & 1 / 1 / 0 / 0 & 1 / 1 / 0 \\
\hline
Maintainability implications & long-term & peer-reviewed & Case study & 2 & 0 / 1 / 0 / 0 & 0 / 1 / 0 / 0 & 0 / 0 / 2 \\
\hline
Maintainability implications & long-term & peer-reviewed & Design proposal or tool description & 1 & 0 / 0 / 0 / 0 & 0 / 1 / 0 / 0 & 0 / 0 / 1 \\
\hline
Maintainability implications & long-term & peer-reviewed & Interviews & 1 & 0 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 0 / 1 / 0 \\
\hline
Maintainability implications & long-term & peer-reviewed & Mixed methods & 1 & 0 / 0 / 1 / 0 & 0 / 0 / 0 / 0 & 0 / 0 / 1 \\
\hline
Maintainability implications & long-term & peer-reviewed & Other & 3 & 0 / 1 / 0 / 0 & 1 / 1 / 0 / 0 & 1 / 2 / 0 \\
\hline
Maintainability implications & long-term & peer-reviewed & Repository mining & 2 & 0 / 2 / 0 / 0 & 0 / 0 / 0 / 0 & 1 / 1 / 0 \\
\hline
Maintainability implications & long-term & peer-reviewed & Static or automated analysis & 1 & 0 / 0 / 0 / 0 & 0 / 1 / 0 / 0 & 0 / 0 / 1 \\
\hline
Maintainability implications & long-term & grey & Conceptual & 3 & 0 / 0 / 0 / 0 & 0 / 3 / 0 / 0 & 0 / 0 / 3 \\
\hline
Maintainability implications & long-term & grey & Empirical & 10 & 1 / 8 / 0 / 1 & 0 / 0 / 0 / 0 & 4 / 5 / 1 \\
\hline
Maintainability implications & long-term & grey & Experience report & 3 & 0 / 0 / 0 / 0 & 0 / 2 / 1 / 0 & 0 / 2 / 1 \\
\hline
Maintainability implications & long-term & grey & Position & 2 & 0 / 0 / 0 / 0 & 0 / 2 / 0 / 0 & 0 / 0 / 2 \\
\hline
Maintainability implications & long-term & grey & Secondary & 3 & 0 / 0 / 0 / 0 & 0 / 3 / 0 / 0 & 0 / 0 / 3 \\
\hline
Maintainability implications & long-term & grey & Tool/System & 3 & 1 / 2 / 0 / 0 & 0 / 0 / 0 / 0 & 1 / 0 / 2 \\
\hline
Reproducibility and consistency & short-term & peer-reviewed & Mixed methods & 1 & 0 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 1 / 0 / 0 \\
\hline
Reproducibility and consistency & short-term & peer-reviewed & Other & 1 & 0 / 0 / 0 / 0 & 1 / 0 / 0 / 0 & 0 / 0 / 1 \\
\hline
Reproducibility and consistency & short-term & peer-reviewed & Static or automated analysis & 1 & 0 / 0 / 0 / 0 & 0 / 1 / 0 / 0 & 0 / 0 / 1 \\
\hline
Reproducibility and consistency & short-term & grey & Conceptual & 1 & 0 / 0 / 0 / 0 & 0 / 1 / 0 / 0 & 0 / 0 / 1 \\
\hline
Reproducibility and consistency & short-term & grey & Empirical & 1 & 0 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 0 / 0 / 1 \\
\hline
Reproducibility and consistency & short-term & grey & Experience report & 1 & 0 / 0 / 0 / 0 & 1 / 0 / 0 / 0 & 1 / 0 / 0 \\
\hline
Reproducibility and consistency & short-term & grey & Tool/System & 1 & 0 / 1 / 0 / 0 & 0 / 0 / 0 / 0 & 1 / 0 / 0 \\
\hline
\end{longtable}
\endgroup


==> tab_safeguard_evaluations_all.tex <==

\begingroup\footnotesize\setlength{\tabcolsep}{4pt}\renewcommand{\arraystretch}{1.1}\captionsetup{font={sf,small},labelfont={bf},labelsep=newline,justification=justified,singlelinecheck=false}
\begin{longtable}{|p{1.1cm}|p{3.0cm}|p{6.0cm}|p{3.2cm}|p{1.8cm}|}
\caption{Safeguards evaluated empirically, with the reported result: every source and coded safeguard whose reporting mode is evaluated (Section~\ref{sec:rq5_2}). Beneficial: the safeguard reduced the risk or improved its target. Mixed: a benefit with a cost or a partial effect. Limiting: the safeguard failed or left the problem in place. Not stated: no separate result. BDD: behavior-driven development. SAST: static application security testing. O-RAN: Open Radio Access Network.}\label{tab:safeguard_evaluations_all}\\
\hline\rowcolor[HTML]{EFEFEF}\textbf{Source} & \textbf{Safeguard} & \textbf{What was evaluated} & \textbf{Design} & \textbf{Result} \\\hline\endfirsthead
\hline\rowcolor[HTML]{EFEFEF}\textbf{Source} & \textbf{Safeguard} & \textbf{What was evaluated} & \textbf{Design} & \textbf{Result} \\\hline\endhead
\ref{WL2} & validation and testing pipelines & syntax checker guard with LLM regeneration (up to 10 trials) & benchmark & not stated \\
\hline
\ref{WL31} & human-in-the-loop review & first author testing and reviewing Cursor output in real time and adjusting prompts & case study & beneficial \\
\hline
\ref{WL61} & human-in-the-loop review & Sustained human control and review of generated code in the MenuCal case & case study & beneficial \\
\hline
\ref{WL63} & human-in-the-loop review & manual check of every LLM-generated file by the authors & case study & not stated \\
\hline
\ref{WL63} & validation and testing pipelines & LPTP proof-checking loop with runtime tests until proofs are certified & case study & mixed \\
\hline
\ref{WL64} & validation and testing pipelines & Static analysis applied to LLM generated backend code & experiment & limiting \\
\hline
\ref{WL68} & validation and testing pipelines & Writing tests, together with versioning, to keep generated code under control & case study & mixed \\
\hline
\ref{WL74} & human-in-the-loop review & interactive decomposition (ANPL) with user-provided input-output checks and execution-trace bug detection & within-subject user study & beneficial \\
\hline
\ref{GL26} & human-in-the-loop review & human review and approval of the plan and of generated code before integration & case study & beneficial \\
\hline
\ref{GL35} & human-in-the-loop review & Ask mode requiring explicit confirmation before the assistant modifies files & user study & beneficial \\
\hline
\ref{GL39} & human-in-the-loop review & mandatory security review processes & benchmark & not stated \\
\hline
\ref{GL54} & validation and testing pipelines & deterministic static checking of user-specified constraints (FlowCheck) in vibe-coded web apps & injected-bug evaluation with formative study & beneficial \\
\hline
\ref{GL55} & human-in-the-loop review & manual security testing alongside automated scanners & controlled twin-prompt generation study & beneficial \\
\hline
\ref{GL55} & validation and testing pipelines & single automated security scanner as the sole check & controlled twin-prompt generation study & limiting \\
\hline
\ref{GL56} & sandboxing and constrained execution & isolation of side effects for parallel agents versus shared state without a merge protocol & benchmark (100 configurations) & beneficial \\
\hline
\ref{GL56} & validation and testing pipelines & framework-side validators checking ports, HTTP behavior and artifacts before accepting completion claims & benchmark (100 configurations) & not stated \\
\hline
\ref{GL57} & human-in-the-loop review & Human involvement in the workflow compared with fully automated runs & experiment & mixed \\
\hline
\ref{GL58} & human-in-the-loop review & structured human validation of LLM code via verifiable literate programming (VLP) with symbolic checking by CrossHair & bug study, simulated-user benchmark and small user study & beneficial \\
\hline
\ref{GL58} & validation and testing pipelines & Automated validation of generated code, including CrossHair symbolic checking, compared with a human and LLM loop & benchmark & mixed \\
\hline
\ref{GL60} & validation and testing pipelines & test feedback passed back to the agent with retry (harness feedback) & benchmark (multi-turn agents) & beneficial \\
\hline
\ref{GL70} & validation and testing pipelines & execution-based Tester agent returning PASS/FAIL feedback for incremental repair, plus multi-layer correctness evaluation & benchmark & not stated \\
\hline
\ref{GL73} & validation and testing pipelines & executable BDD acceptance tests (Robot Framework) fed back to the agent on failure & design science research with exploratory three-condition comparison & mixed \\
\hline
\ref{GL75} & validation and testing pipelines & feedback loop checking generated code against architectural constraints and temporal functional constraints without human inspection & simulated feedback-loop feasibility study & beneficial \\
\hline
\ref{GL76} & validation and testing pipelines & deterministic Contract Auditor monitoring graph state and triggering interventions & benchmark comparison & mixed \\
\hline
\ref{GL79} & validation and testing pipelines & adversarial QA agent (Apollo) demanding test output or CI evidence before accepting claims & multi-project deployment study and benchmark & beneficial \\
\hline
\ref{GL81} & validation and testing pipelines & LLM-generated fault-triggering tests used as a repair signal & benchmark & limiting \\
\hline
\ref{GL85} & validation and testing pipelines & automated constraint-based verification tests whose violation reports are fed back to the LLM & repeated LLM experiments on two example systems & beneficial \\
\hline
\ref{GL87} & human-in-the-loop review & human selection of the better version between iterations under an AI instructor & experiment & beneficial \\
\hline
\ref{GL88} & human-in-the-loop review & human feedback step at the end of each REprompt stage when hallucinations occur, with scope decisions by the interviewer & LLM-judge and human evaluation & not stated \\
\hline
\ref{GL98} & validation and testing pipelines & formal verification of LLM-generated code against human-written specifications (vericoding), with unit tests as a later check & benchmark & mixed \\
\hline
\ref{GL99} & validation and testing pipelines & functional tests as acceptance signal, checked against proof-of-vulnerability tests and SAST & benchmark & limiting \\
\hline
\ref{GL100} & validation and testing pipelines & monitoring of rule violations by other agents in the multi agent configuration & experiment & mixed \\
\hline
\ref{GL120} & human-in-the-loop review & lightweight review of generated code by developers in think aloud videos & user study & not stated \\
\hline
\ref{GL153} & human-in-the-loop review & developer oversight of agents through injected context and behavioural constraints in logged sessions & log analysis & not stated \\
\hline
\ref{GL153} & validation and testing pipelines & AI assisted code checks by static review and runtime inspection, as observed in developer logs & log analysis & not stated \\
\hline
\ref{GL172} & validation and testing pipelines & system-level validation of generated xApps on a real O-RAN testbed, with specification-grounded generation & testbed evaluation with ablation & beneficial \\
\hline
\ref{GL177} & human-in-the-loop review & user confirmation that the formal query matches their intent & benchmark & not stated \\
\hline
\ref{GL177} & validation and testing pipelines & formal verification (Astrogator) of generated programs against a Formal Query Language intent & benchmark & beneficial \\
\hline
\end{longtable}
\endgroup


==> tab_wl_quality_scores_all.tex <==

\begingroup\setlength{\tabcolsep}{4pt}\captionsetup{font={sf,small},labelfont={bf},labelsep=newline,justification=justified,singlelinecheck=false}\begin{longtable}{|p{1.37cm}|p{2.75cm}|p{5.49cm}|p{2.55cm}|p{1.57cm}|p{1.77cm}|}
\caption{Quality assessment of every peer-reviewed source: evidence category, method category, number of applicable checklist items, score as the proportion of applicable items, and band (WL28 scored below 0.50 and is not listed). The checklist measures reporting quality. Empirical rigor is weighted through criterion C2 of the evidence-strength matrix and is not applicable to conceptual and secondary papers.}\label{tab:wl_quality_scores_all}\\
\hline\rowcolor[HTML]{EFEFEF}\textbf{ID} & \textbf{Evidence} & \textbf{Method} & \textbf{Applicable items} & \textbf{Score} & \textbf{Band} \\\hline\endfirsthead
\hline\rowcolor[HTML]{EFEFEF}\textbf{ID} & \textbf{Evidence} & \textbf{Method} & \textbf{Applicable items} & \textbf{Score} & \textbf{Band} \\\hline\endhead
WL1 & Tool/System & Experiment or user study & 9 & 0.83 & High \\\hline
WL2 & Tool/System & Experiment or user study & 9 & 0.85 & High \\\hline
WL3 & Secondary & Review or mapping & 9 & 0.50 & Low \\\hline
WL4 & Empirical & Survey & 10 & 0.95 & High \\\hline
WL5 & Empirical & Survey & 11 & 0.95 & High \\\hline
WL6 & Empirical & Interviews & 10 & 0.70 & Medium \\\hline
WL7 & Tool/System & Case study & 10 & 0.60 & Medium \\\hline
WL8 & Conceptual & Taxonomy or framework & 7 & 0.56 & Low \\\hline
WL9 & Secondary & Static or automated analysis & 9 & 0.50 & Low \\\hline
WL10 & Empirical & Static or automated analysis & 9 & 0.90 & High \\\hline
WL11 & Tool/System & Interviews & 11 & 0.95 & High \\\hline
WL12 & Tool/System & Survey & 11 & 1.00 & High \\\hline
WL13 & Empirical & Experiment or user study & 11 & 0.95 & High \\\hline
WL14 & Conceptual & Static or automated analysis & 7 & 0.71 & Medium \\\hline
WL15 & Conceptual & Other & 6 & 0.75 & High \\\hline
WL16 & Empirical & Interviews & 10 & 1.00 & High \\\hline
WL17 & Tool/System & Case study & 9 & 0.72 & Medium \\\hline
WL18 & Tool/System & Survey & 11 & 0.91 & High \\\hline
WL19 & Empirical & Interviews & 11 & 0.95 & High \\\hline
WL20 & Conceptual & Other & 6 & 0.75 & High \\\hline
WL21 & Secondary & Review or mapping & 8 & 0.81 & High \\\hline
WL22 & Empirical & Survey & 11 & 0.91 & High \\\hline
WL23 & Empirical & Interviews & 11 & 1.00 & High \\\hline
WL24 & Empirical & Other & 10 & 0.65 & Medium \\\hline
WL25 & Conceptual & Static or automated analysis & 9 & 0.61 & Medium \\\hline
WL26 & Tool/System & Taxonomy or framework & 6 & 0.75 & High \\\hline
WL27 & Conceptual & Static or automated analysis & 7 & 0.79 & High \\\hline
WL29 & Empirical & Benchmark & 10 & 0.75 & High \\\hline
WL30 & Empirical & Experiment or user study & 10 & 0.60 & Medium \\\hline
WL31 & Empirical & Case study & 11 & 0.73 & Medium \\\hline
WL32 & Empirical & Case study & 10 & 0.90 & High \\\hline
WL33 & Empirical & Repository mining & 10 & 1.00 & High \\\hline
WL34 & Empirical & Other & 10 & 1.00 & High \\\hline
WL35 & Empirical & Mixed methods & 11 & 0.95 & High \\\hline
WL36 & Empirical & Experiment or user study & 10 & 1.00 & High \\\hline
WL37 & Empirical & Mixed methods & 11 & 0.95 & High \\\hline
WL38 & Position & Design proposal or tool description & 10 & 0.65 & Medium \\\hline
WL39 & Empirical & Mixed methods & 11 & 0.95 & High \\\hline
WL40 & Empirical & Interviews & 11 & 1.00 & High \\\hline
WL41 & Empirical & Repository mining & 9 & 0.94 & High \\\hline
WL42 & Empirical & Repository mining & 10 & 1.00 & High \\\hline
WL43 & Empirical & Repository mining & 10 & 1.00 & High \\\hline
WL44 & Empirical & Mixed methods & 11 & 0.82 & High \\\hline
WL45 & Empirical & Case study & 11 & 0.55 & Low \\\hline
WL46 & Tool/System & Benchmark & 10 & 1.00 & High \\\hline
WL47 & Empirical & Static or automated analysis & 11 & 1.00 & High \\\hline
WL48 & Tool/System & Benchmark & 10 & 1.00 & High \\\hline
WL49 & Empirical & Other & 11 & 0.95 & High \\\hline
WL50 & Empirical & Interviews & 10 & 1.00 & High \\\hline
WL51 & Empirical & Mixed methods & 11 & 1.00 & High \\\hline
WL52 & Conceptual & Design proposal or tool description & 11 & 0.73 & Medium \\\hline
WL53 & Tool/System & Mixed methods & 10 & 0.95 & High \\\hline
WL54 & Empirical & Benchmark & 10 & 0.75 & High \\\hline
WL55 & Empirical & Case study & 11 & 0.95 & High \\\hline
WL56 & Empirical & Mixed methods & 11 & 0.82 & High \\\hline
WL57 & Position & Not reported & 9 & 0.61 & Medium \\\hline
WL58 & Empirical & Interviews & 10 & 0.80 & High \\\hline
WL59 & Empirical & Mixed methods & 11 & 0.55 & Low \\\hline
WL60 & Empirical & Survey & 11 & 0.50 & Low \\\hline
WL61 & Empirical & Case study & 9 & 0.56 & Low \\\hline
WL62 & Empirical & Case study & 11 & 0.73 & Medium \\\hline
WL63 & Empirical & Case study & 10 & 0.80 & High \\\hline
WL64 & Empirical & Mixed methods & 10 & 0.85 & High \\\hline
WL65 & Empirical & Survey & 11 & 0.68 & Medium \\\hline
WL66 & Empirical & Case study & 11 & 0.82 & High \\\hline
WL67 & Tool/System & Design proposal or tool description & 10 & 0.55 & Low \\\hline
WL68 & Empirical & Other & 10 & 0.95 & High \\\hline
WL69 & Empirical & Case study & 10 & 0.85 & High \\\hline
WL70 & Tool/System & Design proposal or tool description & 11 & 0.73 & Medium \\\hline
WL71 & Empirical & Case study & 9 & 0.56 & Low \\\hline
WL72 & Empirical & Mixed methods & 11 & 0.82 & High \\\hline
WL73 & Empirical & Other & 10 & 0.60 & Medium \\\hline
WL74 & Tool/System & Mixed methods & 11 & 0.77 & High \\\hline
WL75 & Position & Other & 5 & 0.70 & Medium \\\hline
WL76 & Empirical & Mixed methods & 11 & 0.82 & High \\\hline
WL77 & Tool/System & Other & 10 & 0.65 & Medium \\\hline
\end{longtable}\endgroup

